RefExpo: Unveiling Software Project Structures through Advanced Dependency Graph Extraction

The dependency graph (DG) of a software project offers valuable insights for identifying its key components and has been leveraged in numerous studies. However, there is a lack of reusable tools for DG extraction. Existing tools are either outdated and difficult to configure or fail to provide accurate analysis. This study introduces RefExpo, a reusable DG extraction tool that supports multiple languages such as Java, Python, and JavaScript. RefExpo is a plugin based on IntelliJ, a well-maintained and reputed IDE. We also compile an initial version of our dataset, consisting of 20 Java and Python projects. RefExpo's validity is evaluated at two levels: specific language features and comparisons against other tools, referred to as micro and macro levels. Our results show RefExpo achieves 92\% and 100\% recall on micro test suites Judge and PyCG for Python and Java, respectively. In macro-level experiments, RefExpo outperformed existing tools by 31\% and 7\% in finding unique and shared results. The installable version of RefExpo is available on the IntelliJ marketplace, and a short video describing its functionality is available on YouTube.

==> sections/callvsdependency.tex <==
In this section, we clarify the distinctions between call graphs and dependency graphs, which is essential for understanding our evaluation method of \tool{}. 
While \tool\ produces dependency graphs, we evaluated its performance against tools that generate call graphs since there are not many updated tools for dependency graphs. 
This explanation aims to elucidate these concepts and justify our evaluation approach.

Call graphs are only concerned about the possible paths and routes that control flow might navigate during execution as a result of function invocation~\cite{ryder-callGraph, ferrante-flowdependency}
In contrast, dependency graphs pay attention to all possible components that are referenced from a component, where method calls are considered as one of them.
Although the definitions might sound simple, there might be some confusion involved.
Code example~\ref{lst:methodReturn} demonstrates a logic where \texttt{func3} obtains an instance of \texttt{func1} by calling \texttt{func2}.
Figure~\ref{fig:callGraph} and Figure~\ref{fig:dependencyGraph} present two possible graphs for this logic.
The difference between these graphs is that one has an edge between \texttt{func3} and \texttt{func1}, and the other one does not.
The most accurate way of constructing call graphs is to evaluate the runtime information~\cite{ryder-callGraph, ferrante-flowdependency}.
Therefore, since this logic will result in a function call from \texttt{func3} to \texttt{func1} during execution, this edge should be included in a call graph.
Hence, Figure~\ref{fig:callGraph} can represent the call graph.
Nevertheless, the dependency graphs are flexible in this regard.
For instance, if one is concerned with coupling evaluation, depending on their scope, they might want to include or remove the dynamic call edges~\cite{briand-coupling}.
Thus, some researchers might find those edges beneficial for their purposes or disturbing~\cite{borowski-semantiGraph}.
If we look at the exact implementation of the logic in Code Example~\ref{lst:methodReturn} in type strict languages, it is more doubtful that such a link should be included. 
Since it works against object-oriented design patterns and creates abstraction. 
Code Example~\ref{lst:interfaceReturn} shows an equivalent implementation of Code Example~\ref{lst:methodReturn} in Java language.
In Java, the language structure suggests the usage of design patterns and interfaces to break this link.
Therefore, in these cases, mining back these links and putting them into the graph might even be a bad idea and be considered as fighting against the language structure.
The language provides all these features to increase the modularity of the code and weaken links between unrelated logic.
Code Example~\ref{lst:judgeDynamicLink} shows a test case example from Judge test suits.
As it is obvious, the method \texttt{castToTarget} is designed to be ignorant about the class type that is passed to it.
Then, tracing back the dependencies and establishing the dynamic links sounds like fighting against a designed principle called separation of concerns~\cite{booch-oop}.
With all said, there is still no general consensus about these dynamic links, and they might not be beneficial for the majority of static code analysis studies.
Considering the complexity of mining dynamic links and the doubt about their usefulness in the context of static code analysis, we choose not to include them in the \tool\ evaluations.

\begin{lstlisting}[language=Python, caption={Python code for method referencing}, label={lst:methodReturn}]
def func1():
    return "Hello from the first function!"

def func2():
    return func1

def func3:
    func = func2()
    print(func())
\end{lstlisting}

\begin{lstlisting}[language=Java, caption={Java code for interface Implementation}, label={lst:interfaceReturn}]
interface Interface {
    void func();
}

class InterfaceImpl implements Interface {
    public void func() {
        System.out.println("Hello World");
    }
}

public static Interface generator() {
    return new InterfaceImpl();
}
    
public static void executeFunc() {
    Interface instance = generator();
    instance.func();
}
\end{lstlisting}

\begin{lstlisting}[language=Java, caption={Java example of dynamic linkage from Judge test suite}, label={lst:judgeDynamicLink}]
static <T> void castToTarget(Class<T> cls,  Object o) {
    T target = cls.cast(o);
    target.toString();
}
\end{lstlisting}


\begin{figure}[ht]
    \centering
    
    \begin{subfigure}[b]{0.45\columnwidth} % Specifies the size of the subfigure
        \centering
        \includesvg[width=\textwidth]{callGraph.svg}
        \caption{Call Graph}
        \label{fig:callGraph}
    \end{subfigure}
    \hfill % Adds space between the subfigures
    \begin{subfigure}[b]{0.45\columnwidth} % Adjust the width as needed
        \centering
        \includesvg[width=\textwidth]{dependencyGraph.svg}
        \caption{Dependency Graph}
        \label{fig:dependencyGraph}
    \end{subfigure}
    
    % Add more subfigures here if needed
    
    \caption{Graphs for example Code~\ref{lst:methodReturn}}
    \label{fig:images}
\end{figure}

==> sections/relatedWorks.tex <==
\subsection{Java Tools}

The majority of existing tools\cite{jarviz, df} providing evaluation specifically for Java, focus on the built artifacts such as JAR or WAR files.
However, we could not find any updated and ready-to-use tool that provides these evaluations from Java source code.
Nevertheless, tools such as Sonargraph\todo{add link} provide these evaluations from source code but they need to build tool configuration to build the artifacts and then provide evaluations.
Besides, tools such as OPAL\todo{add link} require lots of custom implementations and are not ready to use out of the box.

\paragraphTitle{Dependency Finder}
DependencyFinder~\cite{df} is a tool tailored for Java application analysis, focusing on evaluating single artifacts, such as JAR or WAR files. 
Its functionality is centered on a detailed examination of these artifacts, with an emphasis on identifying dependencies within the code. 
Notably, DependencyFinder is capable of detecting method and property accesses, offering a granular view of code interactions. 
Although it has great features to extract and browse dependencies, it comes short in evaluating large projects that produce complex artifacts that are not packed in a single file.

\paragraphTitle{Jarviz}
Jarviz~\cite{jarviz}, a tool designed for Java application analysis, specializes in evaluating JAR files, with the capability to analyze multiple JAR files concurrently. 
However, it requires explicit specification of dependencies for accurate assessment. 
A significant aspect of Jarviz's functionality lies in its ability to detect method-level dependencies within the code, providing insights into the method interactions and dependencies across different JAR files.
Unlike some other tools, Jarviz does not offer features for detecting property accesses unless they are accessed via method calls (getters and setters), focusing instead on method-level analysis.

\paragraphTitle{OPAL}
OPAL~\cite{reif-opal} presents a sophisticated static analysis platform tailored to support developers in optimizing the precision, soundness, and performance of their static analyses.
It is designed to evaluate and decompile Java-compiled outputs such as class files and JAR files and provide the evaluation.
Opal effectively executes the analysis modules to ensure scalability which is one of the main features that scientific tools suffer from.
It does not provide a direct feature for constructing DG, although tracing dependencies is a fundamental feature of any static analysis toolbox.
Hence, it is flexible in the evaluation level based on the custom implementation and can track references in all levels such as class, method, etc.


\paragraphTitle{\tool{}}
The main advantage of \tool\ for Java evaluation is its ease of use.
To use \tool\, no JAR file is required, which does not limit options to small projects.
Moreover, no knowledge of the underlying build mechanism is required since IntelliJ is capable of reading all the structures.
Finally, it evaluates all available files in a given repository and includes test files and other files. 


\subsection{Python Tools}
Generating dependency graphs for Python projects is different for doing that in strictly typed languages, due to the flexibility of the language and allowing runtime reference resolution.
There is no compiled byte code such as a JAR file that contains almost all references specified in the code and all the references are interpreted at runtime.
Although there are dynamic call analysis tools~\cite{callgrind}, this domain has its own challenges regarding static dependency analysis and reference resolution~\cite{sot_js}.

\paragraphTitle{Pyan}
Pyan~\cite{pyan} is a code analysis tool for Python. 
Its performance in tracking classes and functions directly from the source code makes it a key solution in the realm of Python code analysis
However, Pyan has its limitations, particularly in identifying more complex structures such as nested functions or function pointers. 
Besides, the main disadvantage of Pyan is that it supports Python to 3.6.

\paragraphTitle{PyCG}
PyCG~\cite{pycg} represents an additional tool for Python code analysis. 
It provides a new practical way of constructing call graphs and running security vulnerability evaluations by statically analyzing the code with an eye on time efficiency.
It provides a novel way of evaluating a chain of variable assignments and function passing to construct a more accurate call graph.
A notable achievement of PyCG is its remarkable accuracy in call graph generation, achieving a 99.2\% success rate within their specific microsite. 
Additionally, PyCG contributes by offering a micro suite designed to assess the performance of various tools across different aspects of the Python language.
PyCG is only compatible with Python 3.6 and 3.7 and is officially archived.


\paragraphTitle{\tool{}}
A main advantage of \tool\ over other Python-centric tools is the modularity of IntelliJ when it comes to Python interpreter.
IntelliJ can utilize any Python interpreter provided to it which makes it compatible with all Python versions.
However, the main limiting factor of the currently available tools is the version of Python they support. 
Usually, these tools have their intrinsic interpreting logic which limits them to specific versions of Python.
However, 
Therefore, \tool\ can support all the old and new versions of Python.
Another advantage of \tool\ is rooted in its robust foundation, IntelliJ.
Since IntelliJ is backed by an established firm JetBrains and supported by a big community it will be maintained over time which makes \tool\ compatible with feature advancements.
The main disadvantage of \tool\ compared to the previously mentioned tool is its inability to extract dynamic references. These references are not explicitly present in the code but are determined at runtime based on the inputs.

\subsection{Multi-Lingual tools}

\paragraphTitle{Sonargraph}
Sonargraph~\cite{sonargraph} is a software architecture management tool that analyzes the quality of codebases, particularly in \texttt{Java}, \texttt{C\#}, and \texttt{Python} projects. 
A standout feature of Sonargraph is its Dependency Extraction capability. 
This functionality scans the code structure, extracting and visualizing dependencies between packages, classes, and methods. 
It provides second-level evaluations of code dependencies, enabling developers to identify and resolve complex dependency issues, such as cyclic dependencies.
Although it can provide evaluations for Python from source code, for Java projects it has tools that should be configured in build tools, and at the end it evaluates the build results.
This makes it a semi-source-based tool.

\paragraphTitle{\tool{}}
Normally multi-lingual tools demand a good amount of configuration to start their evaluation.
In contrast, \tool\ offers no configuration feature since it can automatically detect all the programming languages that have been used.
Nevertheless, it can provide advanced and framework-related evaluations such as evaluating Angular directives in HTML files upon proper configuration of additional plugins.
Moreover, it can handle different programming languages in a single project which is another limit factor of the mentioned tools.
The modular nature of IntelliJ supports modules with different programming languages or SDKs and also it can support different languages in one module.

